Foundations for Entailment Checking in Quantitative Separation Logic (extended version)

Quantitative separation logic (QSL) is an extension of separation logic (SL) for the verification of probabilistic pointer programs. In QSL, formulae evaluate to real numbers instead of truth values, e.g., the probability of memory-safe termination in a given symbolic heap. As with \SL, one of the key problems when reasoning with QSL is \emph{entailment}: does a formula f entail another formula g? We give a generic reduction from entailment checking in QSL to entailment checking in SL. This allows to leverage the large body of SL research for the automated verification of probabilistic pointer programs. We analyze the complexity of our approach and demonstrate its applicability. In particular, we obtain the first decidability results for the verification of such programs by applying our reduction to a quantitative extension of the well-known symbolic-heap fragment of separation logic.

==> soundness_downward.tex <==
\begin{definition}
	
	
	The set $\SNF$ of quantitative separation logic formulae in \emph{(downward closed) summation normal form} consists of all formulae \mbox{$\ff$ of the form}
	%
	$$ \ff \eeq \sum_{i\in \II} \ra_i \cdot \iverson{\sla_i}~, $$
	%
	where
	\begin{enumerate}
		 \item $\II=\{1,\ldots,n\}$ for some $n\geq 1$ is an index set,
		 %
		 \item $\sla_i \in \SLA$ and $\ra_i \in \NonNegRats$ for all $i \in \II$, and
		 %
		 \item for all $i,j \in \II$ with $i>j$ we have $\sla_i \entails \sla_j$.
	\end{enumerate}
    %
	%
\end{definition}
%
%
%
For $i \in \Nats$, we define $\indexleq{\II}{i}= \{j \in \II ~\mid~ j\leq i\}$. Notice that $\indexleq{\II}{0} = \emptyset$ since $0 \not\in \II$.
The semantics $\sem{\ff}\in \Eone$ of $\ff$ is defined as
%
\[
\semapp{\ff}{(\sk, \hh)} \eeq \sum_{i \in \II} \ra_i \cdot \iverson{\sem{\sla_i}}(\sk,\hh) ~. 
\]
%
%
The set  $\semevaluationSet{\ff} \subset \NonNegRats$ of possible valuations of $\ff$ is given by
%
\[
\semevaluationSet{\ff} \eeq \left\{ \semapp{\ff}{(\sk, \hh)}  ~\mid~ (\sk,\hh) \in  \States \right\}~.
\]
%
Key to our approach is that the \emph{syntactic evaluation set} $\evaluationSet{\ff} \subset \NonNegRats$ given by
%
\[
\evaluationSet{\ff} \eeq \Big\{ \sum_{j\in \indexleq{\II}{i}} \ra_j  ~\mid~ i \in \II \cup\{0\}~, \Big\} ~.
\]
%
%
which soundly overappoximates $\semevaluationSet{\ff}$:
%
\begin{lemma}
	For all $\ff \in \SNF$, we have $\semevaluationSet{\ff} \subseteq \evaluationSet{\ff} $.
\end{lemma}
%
\begin{proof}
	Since $\ff \in \SNF$, we have $\ff = \sum_{i\in \II} \ra_i \cdot \iverson{\sla_i}$. Now let indices of satisfied $\sla_i$ formulae for some state $(\sk, \hh) \in \States$ be $\JJ = \setcomp{i \in \II }{ (\sk, \hh) \models \sla_i }$. Then we have $\sum_{i \in \JJ} \ra_i = \semapp{\ff}{(\sk,\hh)}\in \semevaluationSet{\ff}$. Furthermore, due to downward closeness of $\ff$, we have that if $i \in \JJ$ then $\forall j \leq i~ j \in \JJ$. Now for the maximal index $i\in \JJ$ we have that $\semapp{\ff}{(\sk,\hh)}=\sum_{j \in \JJ} \ra_i = \sum_{j \in \indexleq{\II}{i}} \in \evaluationSet{\ff}$, which proves the lemma.
\end{proof}
%
Notice that $\sizeof{\evaluationSet{\ff}}$ is only linear in the size of $\ff$!
%
%
The at-least construction is much cheaper, too.
%
%
\begin{definition}\label{def:atleast}
	For every $\rb \in \NonNegRats$ and $\ff \eeq \sum_{i\in \II} \ra_i \cdot \iverson{\sla_i} \in \SNF$, we define the $\SLA$ formula $\atleast{\rb}{\ff}$ by
	%
	\begin{align*}
		%    	 \atleast{\ra}{\ff} \quad \eeq \quad \bigvee_{\substack{\JJ \subseteq \II\\ \ra \leq \sum_{j\in \JJ} \rb_j}} ~ \bigwedge_{j \in \JJ} ~ \sla_j ~.
		%    	 \tag*{$\triangle$} \\
		%
		%
		\atleast{\rb}{\ff} \quad \eeq \quad 
		\bigvee_{\{i \in  \II\cup \{0\} ~\mid~ \rb \leq \sum\limits_{j\in \indexleq{\II}{i}} \ra_j \}} ~ \bigwedge_{\substack{ j\in \indexleq{\II}{i}}} ~ \sla_j ~.
		\tag*{$\triangle$}
	\end{align*}
\end{definition}
%
%
Notice that $\sum_\emptyset = 0$ and $\bigwedge_\emptyset \equiv  \true$.
%
%
\begin{lemma}
	Let $\rb \in \NonNegRats$  and $\ff \in \SNF$.
	For all $(\sk,\hh)\in \States$, we have
	%
	$$ \rb \lleq \semapp{\ff}{(\sk,\hh)} \quad\qiff\quad (\sk,\hh) ~{}\models{}~ \atleast{\rb}{\ff} ~.$$
\end{lemma}
\begin{proof}
	We assume $\ff = \sum_{i\in \II} \ra_i \cdot \iverson{\sla_i}$ and let $(\sk, \hh) \in \States$ be an arbitrary states.
	\begin{itemize}
		\item[only:] Let indices of satisfied $\sla_i$ formulae for some state $(\sk, \hh) \in \States$ be $\JJ = \setcomp{i \in \II }{ (\sk, \hh) \models \sla_i }$. Then we have $\rb \leq \sum_{j \in \JJ} \ra_j = \semapp{\ff}{(\sk, \hh)}$. Furthermore by downward closeness of $\ff$ we have some $i' \in \II \cup \{0\}$ such that $\JJ = \indexleq{\II}{i'}$. However, then we can instantiate the index $i$ in \Cref{def:atleast} as the index $i'$.
		\item[if:] Due to $(\sk, \hh) \models \atleast{\rb}{\ff}$, there exists $i\in \II \cup \{0\}$ with $\rb \leq \sum_{j \in \indexleq{\II}{i}} \ra_j$ and for all $j \in \indexleq{\II}{i}$ we have $(\sk, \hh) \models \sla_j$ (thus also $\iverson{\sem{\sla_j}}(\sk, \hh)=1$). Together we have $\rb \leq \sum_{j \in \indexleq{\II}{i}} \ra_j \cdot \iverson{\sem{\sla_j}}(\sk, \hh) \leq \sum_{j \in \II} \ra_j \cdot \iverson{\sem{\sla_j}}(\sk, \hh) = \semapp{\ff}{(\sk, \hh)}$.
	\end{itemize}
\end{proof}
%
%
%
We only need linearly many $\SLA$ entailments:
\begin{theorem}
	For all $\ff, \fg \in \SNF$, we have
	\begin{equation*}
		\ff \entails \fg \qqiff \text{for all}~\ra \in \evaluationSet{\ff}\colon ~ \atleast{\ra}{\ff} \mmodels \atleast{\ra}{\fg} 
	\end{equation*}
\end{theorem}
\begin{proof}

\end{proof}




\subsection{Transforming $\QSLA$ to $\SNF$}



Given a binary operation $\circ \colon \NonNegRats\times\NonNegRats \to \NonNegRats$ and two  sets $V,W \subseteq \NonNegRats$, we define
%
\[
V \circ W
\eeq \big\{ \alpha \circ \beta ~\mid~\alpha \in V ~\text{and}~\beta \in W\big\}~.
\]
%
Furthermore, we write 
%
\[
1-V \eeq \big\{ \Max{0}{1-\rc_{i}} ~\mid~  \rc_{i} \in V \big\} 
%      \end{gather*}
\]
%

%
%
We assume sets of rationals $V$ to be ordered and write $\rc_i \in V$ to indicate that there are $i$ elements in $V$ which are strictly smaller than $\rc_i$. Finally, we often write 
%
\[
\sum_{V }~ (\rc_{i}-\rc_{i-1}) \cdot \ldots
\qquad \text{instead of}\qquad
\sum_{\rc_i, \rc_{i-1} \in V }~ (\rc_{i}-\rc_{i-1}) \cdot \ldots~.
\]
%
For $\ff \eeq \sum_{i\in \II} \ra_i \cdot \iverson{\sla_i} \in \SNF$, $\rb \in \NonNegRats$, and $\BB \in \PurePredset$, we define the shorthands
%
\[
   \rb \cdot \ff \eeq \sum_{i\in \II} (\rb \cdot \ra_i) \cdot \iverson{\sla_i} 
   \quad \text{and}\quad
   \iverson{\BB} \cdot \ff \eeq \sum_{i\in \II} \ra_i \cdot \iverson{\BB \wedge \sla_i } 
\]
%
which are both $\SNF$ formulae.
%
We now define a semantics-preserving transformation $\QSLtoSNFSymbol \colon \QSLA \to \SNF$ according to the rules given in \Cref{tab:QSLtoSNF}.
%
\begin{theorem}[Soundness of translation]\label{thm:SNFTransform}
    For all formulae $\ff \in \QSLA$, 
    \begin{equation*}
      \QSLtoSNF{\ff} \iin \SNF \qquad\text{and}\qquad  \sem{\ff} = \sem{\QSLtoSNF{\ff}}~.
    \end{equation*}
%    where $\QSLtoSNFSymbol: \QSLA \to \SNF$ is defined in \Cref{tab:QSLtoSNF}.
    
\end{theorem}
\kbcommentinline{I propose we prove the cases prob.choice, $\max$ , $\Sup$ ,$\sepcon$ and $\sepimp$ in the paper and provide intuition.}
\subsubsection{Proof of \Cref{thm:SNFTransform}}

\begin{lemma}
	For all formulae $\ff \in \QSLA$ the translation $\QSLtoSNF{\ff}$ is well-typed, that is
	\begin{enumerate}
		\item $\QSLtoSNF{\ff} = \sum_{i \in \II} \ra_i \cdot \iverson{\sla_i}$ with 
		\item $\II=\{1,\ldots,n\}$ for some $n\geq 1$ and
		\item for all $i \in \II~ \ra_i \in \NonNegRats$ and $\sla_i \in \SLA$.
	\end{enumerate}
\end{lemma}
\begin{proof}\ 
	\begin{enumerate}
		\item This holds trivially. \ifcommentinline{Regarding the index sets, this does not really hold...}
		\item Proof by structural induction over $\ff$. The base case holds trivially with $\II = \{1\}$. For the induction step, we can use tha induction hypothesis to conclude that $\II$ in $\QSLtoSNF{\ff} = \sum_{i \in \II} \ra_i \cdot \iverson{\sla_i}$ is finite and nonempty. Then $\evaluationSet{\QSLtoSNFshort{\ff}}$ is also finite and nonempty, as well as $\evaluationSet{\QSLtoSNFshort{\ff}} \circ \evaluationSet{\QSLtoSNFshort{\fg}}$ and $1-\evaluationSet{\QSLtoSNFshort{\ff}}$. Thus the index set after the transformation is also finite and nonempty (and by renaming also $\II=\{1,\ldots,n\}$ for some $n \geq 1$).
		\item Again proof by structural induction over $\ff$. The base case holds again trivially with $\ra_1 = 1$ and $\sla_1 = \preda$. For the induction step, we assume that $\QSLtoSNF{\ff}$ is well-typed.\\
		Since $\NonNegRats$ is closed under addition, multiplication and taking maximum and minimum of two elements, $\Rats$ is closed under $1-\ra$ and $\emax{\ra}{0} \geq 0$, we have that all $\rc_i$ in \Cref{tab:QSLtoSNF} are non negative rational numbers $\rc_i \in \NonNegRats$. Furthermore, we have $\rc_i > \rc_{i-1}$ by to the assumption that the syntactic evaluation sets are ordered sets and $\rc_i$ (resp. $\rc_{i-1}$) has $i$ (resp. $i-1$) many smaller elements in the evaluation set. But then $\rc_i - \rc_{i-1}\in \NonNegRats$ is also non negative and a rational.\\
		Next $\atleast{\rb}{\QSLtoSNFshort{\ff}}$ is an $\SLA$ formulae due the finiteness of the index set of $\QSLtoSNFshort{\ff}$. As already seen above, all syntactic evaluation sets are finite as well. Thus we only have finite combinations of separation logic constructs, which shows that $\sla_i \in \SLA$. 
	\end{enumerate}
\end{proof}

\paragraph{Case} $\pp \cdot \ff + (1-\pp) \cdot \fg$:
\paragraph{Case} $1 - \ff$:
\paragraph{Case} $\emax{\ff}{\fg}$:
\paragraph{Case} $\Sup \xx \colon \ff$:
\paragraph{Case} $\ff \sepcon \fg$:
\paragraph{Case} $\iverson{\preda} \sepimp \ff$:
\ifcommentinline{I need the definition for the semantics here.}

\subsubsection{Transformations without Negation}
\ifcommentinline{These lemmas could be handy in case our SL fragment does not allow negation. But the other transformations perfectly match our syntax. Should we include these nevertheless?}
\begin{lemma}
    Let $\preda, \predb \in \Predset$ and $\ff \in \SNF$. If $\preda \sepcon (\predb \sepimp \false) \equiv \false$, then 
    \begin{equation*}
        \iverson{\preda} \sepcon (\iverson{\predb} \sepimp \ff) \eequiv \sum_{ \evaluationSet{\ff}} (\rc_i - \rc_{i-1}) \cdot \iverson{\preda \sepcon ( \predb \sepimp \atleast{\rc_i}{\ff})}~.
    \end{equation*} 
%
\end{lemma}
\begin{proof}
\ifcommentinline{Finish lemma, also understand this proof}
\end{proof}

\begin{lemma}
    Let $\slsingleton{\xx}{\xy} \in \Predset$ and $\ff \in \SNF$. We have
    \begin{equation*}
    \Inf v \colon \iverson{\slsingleton{v}{\xy}} \sepimp \ff \eequiv \sum_{ \evaluationSet{\ff}} (\rc_i - \rc_{i-1}) \cdot \iverson{\forall v \colon \slsingleton{v}{\xy} \sepimp \atleast{\rc_i}{\ff} }~.
    \end{equation*}
%
\end{lemma}
\begin{proof}
\ifcommentinline{Finish lemma, also complete and understand this proof}
\end{proof}





\begin{table}[th]
	\centering
	\caption{Rules defining the function $\QSLtoSNFSymbol \colon \QSLA \to \SNF$.}
	\label{tab:QSLtoSNF}
	\renewcommand{\arraystretch}{2.0}%
	\begin{tabular}{l@{\qquad\qquad}l@{\qquad}l@{\qquad}l}
		\hline\hline
		$\ff$                                                 & $\QSLtoSNF{\ff}$ \\
		\hline
		$\iverson{\preda}$                                      & 
		$\iverson{\preda}$  \\[1.5em]
		%
		%
		$\iverson{\BB} \cdot \ff +\iverson{\neg\BB}\cdot \fg$                     &
		$\sumInline_{\mathclap{  \evaluationSet{\iverson{\BB}\cdot\QSLtoSNFshort{\ff}}+ \evaluationSet{\iverson{\neg\BB}\cdot\QSLtoSNFshort{\fg}}} }~ (\rc_{i}-\rc_{i-1}) \cdot \big[\bigvee_{\ra \in \evaluationSet{\iverson{\BB}\cdot\QSLtoSNFshort{\ff}}, \rb \in  \evaluationSet{\iverson{\neg\BB}\cdot\QSLtoSNFshort{\fg}}, \ra +\rb\geq \rc_i }
		\atleast{\ra}{\iverson{\BB}\cdot\QSLtoSNFshort{\ff}} \wedge \atleast{\rb}{\iverson{\neg\BB}\cdot\QSLtoSNFshort{\fg}}\big]$\\[1.5em]
		%
		%
		$\pp \cdot \ff + (1-\pp) \cdot \fg$                     &
	$\sumInline_{\mathclap{  \evaluationSet{\pp\cdot\QSLtoSNFshort{\ff}}+ \evaluationSet{(1-\pp)\cdot\QSLtoSNFshort{\fg}}} }~ (\rc_{i}-\rc_{i-1}) \cdot \big[\bigvee_{\ra \in \evaluationSet{\pp\cdot\QSLtoSNFshort{\ff}}, \rb \in  \evaluationSet{(1-\pp)\cdot\QSLtoSNFshort{\fg}}, \ra +\rb\geq \rc_i }
	\atleast{\ra}{\pp\cdot\QSLtoSNFshort{\ff}} \wedge \atleast{\rb}{(1-\pp)\cdot\QSLtoSNFshort{\fg}}\big]$\\[1.5em]
		%
		%
		$\ff \cdot \fg$                                         &
		$\sumInline_{\mathclap{ \evaluationSet{\QSLtoSNFshort{\ff}}\cdot  \evaluationSet{\QSLtoSNFshort{\fg}}} }~ (\rc_{i}-\rc_{i-1}) \cdot \big[\bigvee_{\ra \in \evaluationSet{\QSLtoSNFshort{\ff}}, \rb \in \evaluationSet{\QSLtoSNFshort{\fg}}, \ra\cdot\rb\geq \rc_i }
		\atleast{\ra}{\QSLtoSNFshort{\ff}} \wedge \atleast{\rb}{\QSLtoSNFshort{\fg}}\big]$\\[1.5em]
		%
		%
		$1 - \ff$                                               &
		$\sumInline_{\mathclap{ 1-\evaluationSet{\QSLtoSNFshort{\ff}}} }~ (\rc_{i}-\rc_{i-1}) \cdot \Big[ \atleast{\rc_{i}+\rd-1}{\sumInline_{\mathclap{j \in \indexSet{\ff}}}~ \ra_j \cdot \iverson{{\neg \sla_j}}}\Big]$\\[1.5em]
		%
		%
		$\emax{\ff}{\fg}$                                       &
		$\sumInline_{\mathclap{\evaluationSet{\QSLtoSNFshort{\ff}} \max \evaluationSet{\QSLtoSNFshort{\fg}}}}~ (\rc_{i}-\rc_{i-1}) \cdot \iverson{\atleast{\rc_{i}}{\QSLtoSNFshort{\ff}} \wwedge \atleast{\rc_{i}}{\QSLtoSNFshort{\fg}}}$\\[1.5em]
		%
		%
		$\emin{\ff}{\fg}$                                       &
		$\sumInline_{\mathclap{\evaluationSet{\QSLtoSNFshort{\ff}} \min \evaluationSet{\QSLtoSNFshort{\fg}} }}~ (\rc_{i}-\rc_{i-1}) \cdot \iverson{\atleast{\rc_{i}}{\QSLtoSNFshort{\ff}} \vvee \atleast{\rc_{i}}{\QSLtoSNFshort{\fg}}}$\\[1.5em]
		%
		%
		$\Sup \xx \colon \ff$                                   &
		$\sumInline_{\mathclap{\evaluationSet{\QSLtoSNFshort{\ff}}}}~ (\rc_{i}-\rc_{i-1}) \cdot \iverson{\exists \xx \colon \atleast{\rc_{i}}{\QSLtoSNFshort{\ff}}}$\\[1.5em]
		%
		%
		$\Inf \xx \colon \ff$                                   &
		$\sumInline_{\mathclap{\evaluationSet{\QSLtoSNFshort{\ff}}}}~ (\rc_{i}-\rc_{i-1}) \cdot \iverson{\forall \xx \colon \atleast{\rc_{i}}{\QSLtoSNFshort{\ff}}}$\\[1.5em]
		%
		%
		$\ff \sepcon \fg$                                       &
		$\sumInline_{\mathclap{ \evaluationSet{\QSLtoSNFshort{\ff}}\cdot  \evaluationSet{\QSLtoSNFshort{\fg}}} }~ (\rc_{i}-\rc_{i-1}) \cdot \big[\bigvee_{\ra \in \evaluationSet{\QSLtoSNFshort{\ff}}, \rb \in \evaluationSet{\QSLtoSNFshort{\fg}}, \ra\cdot\rb\geq \rc_i }
			\atleast{\ra}{\QSLtoSNFshort{\ff}} \ssepcon \atleast{\rb}{\QSLtoSNFshort{\fg}}\big]$\\[1.5em]
		%%
		%
		$\iverson{\preda} \sepimp \ff$                          &
		$\sumInline_{\mathclap{ \evaluationSet{\QSLtoSNFshort{\ff}}}}~ (\rc_{i}-\rc_{i-1}) \cdot 
		%            \iverson{\substack{\neg( \preda \substacksepimp \false )\\ 
		%            \land \preda \substacksepimp \atleast{\rc_i}{\QSLtoSNFshort{\ff}}}}$\\[1.5em]
		\iverson{(\neg( \preda \sepimp \false )
			\wwedge \preda \sepimp \atleast{\rc_i}{\QSLtoSNFshort{\ff}}) \vee \iverson{\preda \sepimp \false}}$\\[1.5em]
		%
		%
		\hline\hline
	\end{tabular}%
	\renewcommand{\arraystretch}{1}%
	\\
	where $\QSLtoSNFshort{\ff} = \QSLtoSNF{\ff} = \sum_{i\in \indexSet{\ff}} \ra_i \cdot \iverson{\sla_i}$ , $\QSLtoSNFshort{\fg} = \QSLtoSNF{\fg} = \sum_{j\in \indexSet{\fg}} \rb_i \cdot \iverson{\slb_i}$, and where
	%where $\rc_{i}\in \evaluationSet{\ff}$ is the $i+1$\nth smallest number in $\evaluationSet{\ff}$, 
	$\rd = \sum_{i \in \indexSet{\ff}} \ra_i$.
	% where $\preda \in \Predset$, $\BB \in \PurePredset$, $\neg\BB = \States \setminus \BB$,  $\pp \in [0,1] \cap \Rats$ is a probability,\\
	% and where $\xx \in \Vars$ is a variable.
	% \ifcommentinline{I defined the transformation as a function $\QSLtoSNFSymbol$. We can of course change the symbol. However in my opinion, this symbol makes \Cref{thm:SNFTransform} and \Cref{thm:reducingEntailment} quite neat.}
	%
\end{table}



==> soundness_old.tex <==
\subsection{The Summation Normal Form}

For sake of this proof, we use a mix of $\SLA$ and $\QSLA$ in the form of the \emph{summation normal form}. In these, we allow more then atoms in iverson brackets.

\begin{definition}
A formula $\ff$ is in summation normal form if 
%
$$ \ff \eeq \sum_{i\in \II} \ra_i \cdot \iverson{\sla_i} $$
%
for some non-empty, finite index set $\II$ with $\sla_i \in \SLA$ and $\ra_i \in \NonNegRats$. We denote the set of formulae in summation normal form by $\SNF$. \hfill $\triangle$
%
\end{definition}
%
 We define the semantics $\sem{\ff} \in \Eone$ of a formula $\ff \in \SNF$ in summation normal form by
 %
$$ \semapp{\ff}{(\sk, \hh)} \eeq \sum_{i \in \II} \ra_i \cdot \iverson{\sem{\sla_i}}(\sk,\hh) ~. $$
%
We could restrict the summation normal form to probabilities as coefficients, however, using non-negative rationals is more handy for the later process. If any rational is greater then $1$, the guard is unsatisfiable anyway.
We require to transform an expectation in summation normal form $\ff \in \SNF$ into a separation logic formula that holds exactly when the probability mass exceeds a value $\qq$.

\begin{definition}
	For $\ra \in \NonNegRats$ and $\ff = \sum_{i\in \II} \rb_i \cdot \iverson{\sla_i} \in \SNF$, we define the $\SLA$ formula $\atleast{\ra}{\ff}$ by
	%
    \begin{align*}
%    	 \atleast{\ra}{\ff} \quad \eeq \quad \bigvee_{\substack{\JJ \subseteq \II\\ \ra \leq \sum_{j\in \JJ} \rb_j}} ~ \bigwedge_{j \in \JJ} ~ \sla_j ~.
%    	 \tag*{$\triangle$} \\
    	 %
    	 %
    	 \atleast{\ra}{\ff} \quad \eeq \quad \bigvee_{\{\JJ \subseteq \II ~\mid~ \ra \leq \sum_{j\in \JJ} \rb_j \}} ~ \bigwedge_{j \in \JJ} ~ \sla_j ~.
    	 \tag*{$\triangle$}
    	\end{align*}
\end{definition}

\begin{lemma}
	\label{lem:at_least_sound}
    Let $\ra \in \NonNegRats$  and $\ff \in \SNF$.
    For all $(\sk,\hh)\in \States$, we have
    %
    $$ \ra \lleq \semapp{\ff}{(\sk,\hh)} \quad\qiff\quad (\sk,\hh) ~{}\models{}~ \atleast{\ra}{\ff} ~.$$
\end{lemma}
\begin{proof}
	See \Cref{proof:at_least_sound}.
\end{proof}


%
%
%

\begin{theorem}\label{thm:reducingEntailment}
	For $\ff, \fg \in \QSLA$, we have
	\begin{equation*}
		\ff \entails \fg \qqiff \text{for all}~\ra \in \evaluationSet{\QSLtoSNF{\ff}}\colon ~ \atleast{\ra}{\QSLtoSNF{\ff}} \mmodels \atleast{\ra}{\QSLtoSNF{\fg}} 
	\end{equation*}
\end{theorem}
\begin{proof}
	\ifcommentinline{TODO}
\end{proof}

\kbcommentinline{I am not sure how useful this corollary is for \emph{full} $\QSLA$. Maybe make a theorem out of it and directly talk about fragments fulfilling the requirements  given in \Cref{tab:sla_requirements}? This will be very useful for the applications.}
\begin{corollary}
	Let $\ff, \fg \in \QSLA$ be two formulae in quantitative separation logic and $\QSLtoSNFSymbol: \QSLA \to \SNF$ as defined in \Cref{tab:QSLtoSNF}. $\ff \entails \fg$ is decidable iff $\atleast{\ra}{\QSLtoSNF{\ff}} \models \atleast{\ra}{\QSLtoSNF{\fg}}$ for all $\ra \in \evaluationSet{\QSLtoSNF{\ff}}$ is decidable.
\end{corollary}%
Depending on the syntax that we allow in $\QSLA$, we have different requirements in $\SLA$ to decide entailments in $\QSLA$. An overview for these requirements can be seen in \Cref{tab:sla_requirements}. For the final decision procedure, we use the $\atleast{\ra}{\QSLtoSNF{\ff}}$ transformation, thus all non-trivial operations require both conjunction and disjunction.

\subsection{Transforming $\QSLA$ to $\SNF$}

\ifcommentinline{I suggest defining all evaluation sets we will require here once, so that in the next pages, we do not need to include them every time (although a refresher will be given nevertheless.)}
%
\begin{definition} Let $\ff = \sum_{i\in \indexSet{\ff}} \ra_i \cdot \iverson{\sla_i}$ and $\fg = \sum_{i\in \indexSet{\fg}} \rb_i \cdot \iverson{\slb_i}$ be $\SNF$ formulae. We define the \emph{evaluation set} $\evaluationSet{\ff} \subset \NonNegRats$ of $\ff$ by
%
    \begin{align*}
        \evaluationSet{\ff} \eeq \Big\{\sum_{j\in \JJ} \ra_j ~\mid~\JJ \subseteq \indexSet{\ff} \Big\}~.\tag*{$\triangle$}
    \end{align*}
    %
    %
\end{definition}
%
Notice that for every $\ff$ we have $0 \in \evaluationSet{\ff}$ since $\emptyset \subseteq \II_f$.

    Given a binary operation $\circ \colon \NonNegRats\times\NonNegRats \to \NonNegRats$ and two  sets $V,W \subseteq \NonNegRats$, we define
    %
    \[
        V \circ W
        \eeq \big\{ \alpha \circ \beta ~\mid~\alpha \in V ~\text{and}~\beta \in W\big\}~.
    \]
    %
    Furthermore, we write 
    %
    \[
%       \begin{gather*}
       1-V \eeq \big\{ \Max{0}{1-\rc_{i}} ~\mid~  \rc_{i} \in V \big\} ~.
 %      \end{gather*}
    \]
    %
    %
   If  $V$ has at least $i+1$ elements, we write $\rc_i \in V$ to indicate that $\rc_i$ is the $(i+1)$th smallest element of $V$. Finally, for $\sizeof{V}\geq 2$, we often write 
    %
    \[
         \sum_{V }~ (\rc_{i}-\rc_{i-1}) \cdot \ldots
         \qquad \text{instead of}\qquad
         \sum_{\rc_i, \rc_{i-1} \in V }~ (\rc_{i}-\rc_{i-1}) \cdot \ldots
    \]
    %
    for the sake of convenience.
    %
  \begin{lemma}
  	For all $\ff \in \SNF$ and $(\sk,\hh) \in \States$, we have $\semapp{\ff}{(\sk,\hh)} \in \evaluationSet{\ff}$.
%  	%
%  	\[
%  	\text{for all}~(\sk,\hh) \in \States\colon \quad 
%  	\semapp{\ff}{(\sk,\hh)} ~{}\in{}~ \evaluationSet{\ff}~.
%  	%
%  	\]
  \end{lemma}
%
%
%    Furthermore, we can apply $1-$ to the evaluation set as
%    \begin{gather*}
%        \funcEvaluationSet{1-}{\ff} \eeq \setcomp{ \Max{0}{1-\rc_{i}} }{ \rc_{i} \in \evaluationSet{\ff}} ~,\\
%    \end{gather*}
%    apply $\min$ and $\max$ to it as
%    \begin{gather*}
%        \funcEvaluationSet{\min}{\ff, \fg} \eeq \setcomp{ \Min{\sum_{j\in \JJ} \ra_j}{\sum_{j\in \JJ'} \rb_j} }{ \JJ \subseteq \indexSet{\ff}, \JJ' \subseteq \indexSet{\fg} }~,\\
%        \funcEvaluationSet{\max}{\ff, \fg} \eeq \setcomp{ \Max{\sum_{j\in \JJ} \ra_j}{\sum_{j\in \JJ'} \rb_j} }{ \JJ \subseteq \indexSet{\ff}, \JJ' \subseteq \indexSet{\fg} }~,\\
%    \end{gather*}
%    and apply multiplication to $\evaluationSet{\ff}$ and $\evaluationSet{\fg}$ as
%    \begin{gather*}
%        \funcEvaluationSet{\times}{\ff, \fg} \eeq \setcomp{ \sum_{j\in \JJ} \ra_j \cdot \sum_{j\in \JJ'} \rb_j }{ \JJ \subseteq \indexSet{\ff}, \JJ' \subseteq \indexSet{\fg} } ~.
%    \end{gather*}
%    Whenever we pick an evaluation $\rc_{i} \in \evaluationSet{\ff}$, we assume that $\rc_{i}$ is the $i+1$\nth smallest number in $\evaluationSet{\ff}$.
%\end{definition} %
%%
Remark that we will use these sets in telescoping sums. By combining all neighboring evaluations $\rc_{i-1}, \rc_{i}$ with index smaller or equal then $k$, we can pick exactly $\rb_k$ due to $\rb_0=0$: 
$$\sum_{\rb_{i-1}, \rb_{i} \in \evaluationSet{\ff}, i\leq k} \rb_{i}-\rb_{i-1} \eeq \rb_{k}-\rb_{0} \eeq \rb_{k}~.$$
We can transform a formula in $\QSLA$ into $\SNF$ using the function $\QSLtoSNFSymbol$ defined in \Cref{tab:QSLtoSNF}.
